Why Prototypes Collapse: Diagnosing and Preventing Partial Collapse in Prototypical Self-Supervised Learning

Prototypical self-supervised learning methods consistently suffer from partial prototype collapse, where multiple prototypes converge to nearly identical representations. This undermines their central purpose -- providing diverse and informative targets to guide encoders toward rich representations -- and has led practitioners to over-parameterize prototype sets or add ad-hoc regularizers, which mitigate symptoms rather than address the root cause. We empirically trace the collapse to the joint optimization of encoders and prototypes, which encourages a type of shortcut learning: early in training prototypes drift toward redundant representations that minimize loss without necessarily enhancing representation diversity. To break the joint optimization, we introduce a fully decoupled training strategy that learns prototypes and encoders under separate objectives. Concretely, we model prototypes as a Gaussian mixture updated with an online EM-style procedure, independent of the encoder's loss. This simple yet principled decoupling eliminates prototype collapse without explicit regularization and yields consistently diverse prototypes and stronger downstream performance.

==> sections/0_abstract.tex <==
\begin{abstract}
Although prototypical self-supervised learning frameworks achieve impressive results on curated benchmarks, their performance deteriorates in real-world, in-the-wild settings characterized by long-tailed distributions and pronounced intra-class variability. Extensive experiments reveal that this decline stems from the joint interaction between encoders and prototypes during training. Early on, prototypes shortcut the loss by aligning exclusively with head-class representations, thereby neglecting the embeddings necessary to model tail classes effectively. To address this, we propose \METHODFULLNAME (\METHODNAME), which decouples prototype updates from encoder training by modeling prototypes as components of a dynamic mixture model and updating them via an EM-style procedure that operates independently of the encoder’s objective. This decoupling solves partial collapse, encourages balanced prototype utilization across both head and tail classes, and significantly enhances the model’s capacity to represent underrepresented tail classes for data found in the wild, outperforming existing prototypical SSL methods. Comprehensive evaluations on long-tailed and uncurated datasets demonstrate that \METHODNAME delivers improvements in both robustness and downstream accuracy over existing prototypical SSL methods.
\end{abstract}
% Prototypically based self-supervised learning frameworks often rely on a tightly coupled interplay between encoders and prototypes. We found that the DINO-family of models suffers from prototype collapse, and this problem exacerbates on real-world data where classes are not balanced (in contrast to the curated training setup). A phenomenon we term degenerate collaboration: encoders and prototypes inadvertently collaborate to satisfy the training objective while neglecting the goal of learning truly diverse and discriminative representations.
% To counteract this collapse, we decouple the learning objectives of prototypes and encoders. We proposed \METHODFULLNAME, an EM-based update for prototypes that directly models the data distribution, while the encoder is trained independently via a consistency objective. This separation prevents prototypes from converging on a narrow subset, resulting in more robust representations, higher prototype utilization, and improved downstream performance.
% We verify that our proposal improves the prototype collapse by evaluating models in a long-tail setup through different downstream tasks, as well as through the quantification of the collapsed prototypes.


==> sections/1_introduction.tex <==
\section{Introduction}
Self-supervised learning (SSL), led by prototypical methods in the visual domain~\citep{dinov3}, now rivals the effectiveness of language-supervised alternatives in representation learning~\citep{fan2025webdino}. 
While effective, recent work has demonstrated that many prototypical SSL approaches suffer from a phenomenon known as \textit{partial prototype collapse}, in which multiple prototypes converge to similar representation \citep{govindarajan2023dino, Govindarajan_2024_BMVC}. This phenomenon could explain why over-parameterizing the number of prototypes used have been a popular choice to improve performance in recent prototypical frameworks \citep{oquab2024dinov, dinov3}. While recent efforts have attempted to address this issue through either explicit regularization~\citep{Govindarajan_2024_BMVC, wen2024makes} or implicit mechanisms~\citep{silva2023carp}, the problem remains unresolved, and its underlying causes remain largely unexplored.


In this work, we investigate whether the common practice of jointly optimizing the encoder and prototypes in prototypical SSL frameworks may contribute to the emergence of partial prototype collapse. Intuitively, this joint optimization may allow prototypes to converge toward redundant representations early in training, exploiting shortcuts that minimize the loss but hinder the development of diverse and semantically meaningful representations. This is problematic, 


as effective prototype utilization has been shown to be particularly important for handling data in-the-wild and its long-tailed distributions~\citep{Govindarajan_2024_BMVC, wen2024makes}, a finding we validate through our extensive experiments.

We propose Mixture-Augmented Prototypical Learning (MAPL), a method that decouples the joint optimization of the encoder and prototypes by modeling the prototypes as parameters of a mixture of Gaussians, updated via an EM-style algorithm independently of the encoder’s objective. In our experiments, \textit{we observe no signs of partial collapse}, despite the absence of explicit regularization to maintain prototype diversity~\citep{wen2024makes,Govindarajan_2024_BMVC}. Moreover, MAPL consistently achieves high prototype utilization, demonstrates robustness to mini-batch class imbalance~\citep{assran2023pmsn}, and maintains a diverse set of prototypes compared to existing prototypical methods. We show that MAPL is particularly well-suited for training on long-tailed datasets, while remaining competitive with comparable state-of-the-art methods on class-balanced benchmarks—without the need for manual adjustment of the loss function to adapt to varying data distributions \citep{assran2023pmsn}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/teaser_figure_placeholder.png}
    \caption{a) Traditional joint-embedding architectures with a prototypical formulation: encoders and prototypes are optimized jointly under the same loss, which can lead to shortcut learning and prototype collapse—prototypes converge to similar representations, reducing the effective representation space. (b) Our proposed solution: decouple the gradient flow to the prototypes and train them with a separate objective, mitigating shortcut learning and preserving prototype diversity.}
    \label{fig:placeholder}
\end{figure}

==> sections/2_case_study.tex <==
\section{Understanding Partial Prototype Collapse}
\subsection{Preliminaries}
\citet{Govindarajan_2024_BMVC} investigated the DINO-family of methods \citep{caron2021emerging, zhou2022image, assran2022msn, assran2023pmsn} and demonstrated that these prototypical SSL approaches are susceptible to \textit{partial prototype collapse}. This phenomenon arises when multiple prototypes converge to nearly identical representations during training. While this behavior does not amount to a complete collapse of all prototypes, it nevertheless reduces the diversity of representations and may hinder the effectiveness of downstream tasks. To formalize this behavior, the authors introduced Definition \ref{def:partial_collapse}. Applying this definition, they further showed that the DINO-family of methods retained only about 2–40\% of their initially initialized prototypes as unique, thereby revealing a substantial redundancy in the learned representations. To alleviate this issue, they proposed applying KoLeo regularization \citep{beirlant1997nonparametric, delattre2017kozachenko, sablayrolles_spreading_vectors} directly to the prototypes, introducing an additional objective in the overall loss function to preserve prototype diversity throughout training. 

\begin{definition}[Partial prototype collapse]
\label{def:partial_collapse}
Consider the set $C = \{c_k : k=1,...,K\}$ of $K$ prototype vectors, $c_k$ such that $\Vert c_k \Vert = 1$. A \emph{partial prototype collapse} (of degree $M$ and $\epsilon$ distance) is said to have occurred if there exists a set of $M$ disjoint partitions of prototype vectors $V_m \subset C$, $m = 1, ..., M$, and $M$ representative prototype vectors $v_m \in V_m$, such that for all $m = 1, ..., M$, 
$1-v_m^{\mathsf{T}}c_j < \epsilon$, for all $c_j \in V_m$.
The set of $M$ \emph{unique prototypes} is defined as $U = \{v_m \}_{m=1}^M$.
\end{definition}

\citet{Govindarajan_2024_BMVC} provides an important first step toward understanding the issue of partial prototype collapse. However, their study also leaves several important questions. First, is partial prototype collapse confined to the DINO-family of methods, or does it also occur in other prototypical SSL formulations? Second, at what stage of training does partial prototype collapse emerge, and how does regularization influence its progression? Third, beyond explicitly imposing a regularization term in the loss, are there alternative mechanisms that can encourage and sustain prototype diversity throughout training?


\subsection{Partitioning strategies mitigates prototypical collapse}
\cite{wen2024makes} investigated why CLIP models \citep{radford2021CLIP}, unlike supervised methods, exhibit notable resilience to long-tailed pre-training distributions. Their analysis showed that a key factor behind this robustness is CLIP’s behavior as a dynamic classifier: instead of simultaneously considering the entire set of classes, each mini-batch only involves a subset. Inspired by this mechanism, the authors asked whether DINO—a prototypical SSL method in which all prototypes, analogous to supervised classes, are always active—could similarly benefit from subsampling. By introducing a prototype subsampling strategy, they were able to mitigate partial prototype collapse and improve DINO’s robustness under imbalanced data conditions.

Their subsampling strategy bears a close resemblance to CARP’s \citep{silva2023carp} \textit{random partitioning} approach. In CARP, prototypes are divided into multiple random subsets at each iteration, and consistency is enforced within every subset. This design stabilizes training compared to earlier methods such as CARL \citep{silva2022carl}, allowing CARP to avoid additional collapse-prevention mechanisms. While subsampling and random partitioning share the intuition of reducing the effective prototype space, the key difference is that subsampling uses only a single subset per iteration, whereas CARP leverages all subsets simultaneously. As a result, random partitioning provides an arguably richer supervisory signal, since multiple classification subproblems are posed in parallel at each training step.

In light of this, we pose the question: does the random partitioning strategy, originally introduced in CARP to stabilize training, also help mitigate the partial prototype collapse problem? To investigate this, and to better understand the interaction between prototype collapse and training dynamics, we track the number of unique prototypes in use and the linear evaluation accuracy on ImageNet-1k \citep{deng2009imagenet} over the first 100 epochs for CARL, CARP, DINO, DINO + KoLeoProto, and DINO + Subsampling, as depicted in Figure \ref{fig:protos-acc-two-subplots}. 

A first observation is that partial prototype collapse emerges very early in training: after only 10 epochs, nearly two-thirds of the prototypes have already collapsed. Introducing the KoLeo-Proto (KP) regularizer proves effective at maintaining prototype diversity, underscoring its role as a strong collapse-prevention mechanism. While DINO+KP exhibits a modest drop in accuracy during the early stages of training, this effect diminishes over time, and the final model slightly outperforms vanilla DINO. This suggests that preserving higher prototype diversity throughout training ultimately leads to stronger representations in the converged model.

Another noteworthy observation is that CARP, as hypothesized, is far less prone to prototype collapse than the baseline CARL. By the end of training, CARL retains only about $0.2\%$ of its initialized prototypes as unique, whereas CARP preserves $91.7\%$. This difference is also reflected in linear evaluation performance: CARP consistently outperforms CARL both early and late in training. While these gains cannot be attributed solely to prototype uniqueness—training stability likely plays a significant role—they nevertheless amount to a substantial margin of roughly 3.5 percentage points in linear accuracy by the end of training.

Lastly, we observe that DINO with Subsampling (SS) does alleviate the partial prototype collapse problem to some extent. However, the resulting increase in prototype diversity is accompanied by a considerable drop in accuracy, likely because only a quarter of the prototypes are updated at each iteration, reducing the overall training signal. This suggests that the SS strategy may be more beneficial in settings with uncurated, imbalanced data than on curated, uniform datasets such as ImageNet-1k.



\subsection{Do all prototypical SSL formulations exhibit partial prototype collapse?}
Building on the insights from our previous experiments, we now ask: do other prototypical SSL formulations mitigate partial prototype collapse without relying on explicit regularization terms in the loss or on a partitioning strategy? To address this, we conduct a straightforward experiment in which we download the officially released weights of several prominent prototypical methods and evaluate the diversity of their learned prototypes using various choices of $\epsilon$ from Definition~\ref{def:partial_collapse}. Intuitively, as the threshold $\epsilon$ increases, a higher count of unique prototypes $M$ reflects greater prototype diversity at the end of training.

Observing the results in Table \ref{tab:protos_under_diff_eps} we find that CARP maintain a high prototype utilization, which can be attributed to its partitioning strategy. Somewhat surprisingly, we find that CAPI \citep{darcet2025capi} maintains a high prototype diversity, almost showcasing full uniqueness with only 1 collapsed prototype out of 16,384 for $\epsilon=0.025$. This begs the question, what mechanism in CAPI allows the prototypes to remain diverse throughout training? 

A key distinction of CAPI compared to earlier prototypical joint-embedding frameworks lies in how the teacher’s prototypes are handled. In most prototypical formulations, and in particular the DINO-family, the prototypes used to compute soft assignments for the teacher are an EMA-updated version of the prototypes used for the student, so that the teacher and student prototypes remain tightly coupled through a joint optimization  objective. However, \cite{darcet2025capi} argues that in an masked image modelling (MIM) setting as in iBOT \citep{zhou2022image}, this creates a distributional mismatch: the targets from the teacher’s prototype assignments are made on unmasked patches, while the student's prototype assignments are made on masked patches. They argue that this joint optimization with a distribution mismatch produces instabilities in training. 

CAPI resolves this by decoupling the teacher’s prototypes from the main loss. The teacher encoder generates latent patch embeddings that are assigned to prototypes learned independently within a separate clustering module, and these assignments are then used as the student’s targets. The student branch, in turn, predicts these assignments using its own prototypes, which continue to be updated jointly through the prediction objective. 

Based on the behavior observed in CAPI, we hypothesize that partial prototype collapse in prototypical SSL stems primarily from updating the prototypes and encoders under a shared loss. When prototypes are optimized jointly with the encoder, they may drift toward similar representations that reduce the prediction error without improving the underlying features—a form of shortcut learning. This mechanism helps to explain our findings in Figure \ref{fig:protos-acc-two-subplots}(a), which show that prototypical formulations such as DINO exhibit a large fraction of prototype collapse within the first few epochs of training. Conversely, decoupling the teacher’s prototypes from the main loss, as in CAPI, should reduce this incentive, leading to more stable and diverse prototype usage throughout training.

\begin{table}[ht]
    \centering
    \caption{Unique prototypes for different values of $\epsilon$.}
    \label{tab:protos_under_diff_eps}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l l l l l l l}
        \toprule
        \textbf{Model} & \textbf{Arch} &  \textbf{Objective} &$\boldsymbol{\epsilon = 0.50}$ & $\boldsymbol{\epsilon = 0.25}$ & $\boldsymbol{\epsilon = 0.10}$ & $\boldsymbol{\epsilon = 0.05}$ & $\boldsymbol{\epsilon = 0.025}$ \\
        \midrule
        DINO      & ResNet-50 & Instance &442 (0.7\%) & 791 (1.2\%) & 895 (1.3\%) & 948 (1.4\%) & 1012 (1.6\%) \\
        CARP      & ResNet-50 & Instance &490 (0.7\%) & 1609 (2.5\%) & 5031 (0.8\%) & 10312 (15.7\%) & 19417 (29.6\%) \\
        MSN & ViT-S/16 & Instance  & & & & & 810 (79.1\%) \\
        \midrule
        CAPI & ViT-L/16 & Dense & 9214 (56.2\%) & 14488 (88.4\%) & 16183 (98.8\%) & 16370 (99.9\%) & 16383 (100\%) \\
        \midrule    
        iBOT      & ViT-S/16 & Hybrid  & & & & & 3332 (40.7\%) \\
        iBOT-vMF + KP & ViT-S/16 & Hybrid &-- & -- & -- & -- & 7895 (96.4\%) \\
        Franca & ViT-L/14 & Hybrid & -- & -- & -- & -- & -- \\
        DiNOv2 & ViT-L/14 & Hybrid & -- & -- & -- & -- & -- \\
        DiNOv3 & ViT-7B/16 & Hybrid & -- & -- & -- & -- & -- \\
        \midrule
        \textcolor{gray}{MAPL} & \textcolor{gray}{ResNet-50} & \textcolor{gray}{65536 (100\%)} & \textcolor{gray}{65536 (100\%)} & \textcolor{gray}{65536 (100\%)} & \textcolor{gray}{65536 (100\%)} & \textcolor{gray}{65536 (100\%)} \\
        \bottomrule
    \end{tabular}%
    }
\end{table}





%% TO Revise just remember to mention somwhere
Orthogonal to this line of work, other studies have explored discarding the idea of learning prototypes altogether. However, as \cite{caron2020swav} demonstrated, keeping prototypes fixed leads to subpar performance. Instead, this research direction has shown that, rather than learning prototypes directly, one can maintain a memory bank of the encoder’s past representations to supplement or replace traditional prototypes \citep{gidaris2021obow,gidaris2024moca,silva2024massl,silva2025selforganizing}. This approach can effectively address the partial prototype collapse problem, provided that the stored representations remain diverse and that the encoder itself does not collapse to a trivial solution.


% \begin{figure}[ht]
%     \label{fig:training_dynamics}
%     \centering
%     % First subplot: figure
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \includegraphics[width=\linewidth]{images/Placeholder_unique_protos.png}
%         \caption{Unique prototypes per 10-epoch interval}
%         \label{fig:unique}
%     \end{subfigure}
%     \hfill
%     % Second subplot: table
%     \begin{subfigure}{0.49\linewidth}
%         \centering
%         \begin{tabular}{l c c}
%             \toprule
%             \textbf{Model} & \textbf{Arch }& \textbf{Unique Prototypes} \\
%             \midrule
%             DINO      & ResNet-50 & 1012 (1.6\%) \\
%             iBOT      & ViT-S/16 & 3332 (40.7\%) \\
%             CARP      & ResNet-50   & 19417 (29.6\%) \\
%             CAPI      & ViT-L/16  & 16383 (100\%) \\
%             MSN       & ViT-S/16 & 810 (79.1\%) \\
%             iBOT-vMF + KP & ViT-S/16 & 7895 (96.4\%) \\
%             \bottomrule
%         \end{tabular}
%         \caption{Unique prototypes across models}
%         \label{fig:proto-table}
%     \end{subfigure}
%     \caption{\textbf{PLACEHOLDER:} (a) Comparison of unique prototypes throughout training of DINO, DINO+KP and CARP.(b) Unique prototypes using official weights, as can be seen, CAPI which decouples the training objective from the prototypes maintains a high number of unique prototypes.}
%     \label{fig:prototypes}
% \end{figure}




==> sections/3_method.tex <==
\section{method}
\subsection{Background: Prototypical Self-Supervised Methods}
\label{backgorund:proto_ssl}
To facilitate a formal comparison, we first present a unified view of the methods. Given $V$ stochastic augmentations $\{v_i^{j}\}_{j=1}^V$ of an image $x_i$, the student encoder $f_\theta$ and the EMA-updated teacher $f_\phi$ produce feature vectors that a projection head $g$ maps to representations $h_i^j = g(f_{(\cdot)}(v_i^j ))\in\mathbb{R}^D$.
Similarity scores $z_i^j=C^\top h_i^j\in\mathbb{R}^{K}$ are then computed against a learnable prototype set $C=[c_1 \; c_2 \; \cdots \;c_K]\in\mathbb{R}^{D\times K}$.  All investigated methods translate these scores into a probability distribution over prototypes with an (optionally tempered) softmax operation 
\begin{equation}
p(z_i^j;\tau)=\operatorname{softmax}\!\bigl(z_i^j/\tau\bigr),\qquad \tau>0,
\end{equation}
where $\tau$ is a temperature that controls the sharpness of the distribution; DINO employs a different $\tau<1$ for the student and teacher encoder to sharpen predictions while in CARL and CARP the temperature is fixed at $\tau=1$. Let $P^t, P^s \in \mathbb{R}^{B \times V \times K}$ denote the resulting prototype probability distributions for the teacher and student networks, respectively, where $B$ is the batch size and $V$ the number of augmented views per image. In DINO, the learning objective promotes consistency between the student and teacher outputs across different views of the same image. This is achieved by minimizing the \emph{cross-entropy} between the teacher's distribution for one view and the student's distribution for another, averaged over all distinct pairs of views:
\begin{equation}
    \mathcal{L}_{\text{CE}}(P^t, P^s)= -\frac{1}{B(V-1)} \sum_{i=1}^{B} \sum_{\substack{j,j'=1 \\ j \neq j'}}^{V} P_{i,j}^{t}  \log P_{i,j'}^{s}.
\end{equation}
Similarly, CARL and CARP also enforce consistency between the student and teacher outputs across different views; however, they adopt a \emph{cluster loss} defined as:
\begin{equation}
\label{eq:cluster_loss}
    \mathcal{L}_{\text{CL}}(P^t, P^s) =\frac{1}{B(V-1)} \sum_{i=1}^{B} \sum_{\substack{j,j'=1 \\ j \neq j'}}^{V} -\log \langle P_{i,j}^{t},  P_{i,j'}^{s}\rangle,
\end{equation}
where $\langle \cdot, \cdot \rangle$ denotes the inner product between probability vectors. 
The methods differ in their strategies for avoiding trivial solutions. CARL and CARP incorporate an entropy maximization term over the batch-averaged student and teacher assignments, encouraging uniform prototype usage and preventing the collapse of representations onto a few prototypes. CARL relies on a scheduled regularization strength to balance the consistency and entropy terms, whereas CARP removes this dependency by introducing a \emph{random partitioning} strategy. By partitioning the prototypes into random subsets at each iteration, CARP stabilizes training and eliminates the need for tuning the entropy coefficient. An additional benefit of the random partitioning scheme is an increase in effective prototype utilization, as we demonstrate in Section~\ref{sec:exploration_part}.

% In contrast, DINO prevents trivial collapse by applying a centering operation to the teacher logits before softmax normalization. Subsequent work has shown that replacing centering with Sinkhorn-Knopp normalization~\cite{cuturi2013sinkhorn} further improves prototype utilization~\cite{ruan2023weighted}, a modification adopted as the standard in DINOv2~\cite{oquab2024dinov}. Accordingly, for the remainder of this paper, we replace the centering operation in DINO with Sinkhorn-Knopp normalization.
%% TODO: Go over this paragraph and check for redunancies with sharpening.

\subsection{\METHODFULLNAME (\METHODNAME)}
\label{sec:method}
We hypothesize that the primary cause of partial collapse in prototypical SSL frameworks stems from the joint optimization of the encoder and the prototypes. This intertwined optimization process can lead to an undesirable shortcut, where prototypes converge to similar regions in feature space which simplifies the encoder's task of making assignments and thus minimizing the loss. As demonstrated in Section~\ref{sec:exploratory_part}, this partial collapse emerges relatively early during training. This early collapse is particularly problematic when training on imbalanced (long-tailed) datasets, as prototypes tend to favor features from more frequently occurring classes while neglecting those from less represented classes. In our empirical results, see Section~\ref{sec:experiments}, we showcase that improved prototype utilization directly correlates with increased robustness and enhanced performance when pre-training on long-tailed datasets collected in the wild.


To address the issue of partial collapse arising from joint prototype and encoder optimization, we introduce \METHODFULLNAME (\METHODNAME), a self‑supervised training framework that decouples the joint optimization of prototypes, preventing partial collapse and encouraging high prototype utilization for robust learning. In \METHODNAME, prototypes are parameterized as components of a probabilistic mixture model and updated through an EM‑style procedure. This strategy separates the otherwise joint optimization: rather than directly updating prototypes via backpropagation with respect to the loss, we instead update them by maximizing the data likelihood of teacher embeddings. While the prototypes are updated through this modified procedure, the encoder maintains the established prototypical SSL learning framework detailed in Section~\ref{backgorund:proto_ssl}, leveraging the cluster loss~\eqref{eq:cluster_loss}~\citep{silva2022carl, silva2023carp}, which empirically yields superior results compared to the cross-entropy loss formulation. For further details, refer to the ablations presented in Section~\ref{sec:ablations}.



\subsection{Decoupling the Optimization: Online Gaussian Mixture Model}
To decouple the joint optimization of the encoder and prototypes, we choose to represent prototypes explicitly as components of a Gaussian Mixture Model (GMM). Under this probabilistic formulation, prototypes capture the underlying structure of the data distribution independently from the encoder's training objective. By leveraging an Expectation-Maximization (EM)-based approach~\cite{dempster1977maximum}, prototypes maximize the data likelihood of the teacher's latent embeddings, thereby effectively disentangling their update mechanism from the encoder's loss-driven gradient updates. This separation ensures that prototype optimization is solely governed by the statistical characteristics of the latent representations, promoting robust learning and preventing partial collapse. 

While the classical EM algorithm provides a principled framework for prototype learning, it assumes access to a static and complete dataset. This assumption is incompatible with our SSL framework, where data becomes available incrementally as the encoder continuously updates its representations during training. To address this limitation, we propose to adopt an online variant of the EM algorithm~\cite{neal1998view, sato2000line},  which updates the mixture parameters incrementally using mini-batches of data.  

At each iteration $t$, we treat the incoming batch as a sample from the evolving feature distribution and perform a two-step update: computing responsibilities for each latent vector, followed by an update of the GMM parameters using sufficient statistics.

The GMM is parameterized by $\Psi^{(t-1)} = \{\pi^{(t-1)}, \mu^{(t-1)}, \Sigma^{(t-1)}\}$, where $\pi$, $\mu$, and $\Sigma$ denote the mixture weights, means (prototypes), and diagonal covariances, respectively. For each input $i$, the responsibilities $\gamma_{ik}^{(t)}$ are defined as:
\begin{equation}
    \label{responsibilities}
    \gamma_{ik}^{(t)} = \frac{\pi_k^{(t-1)}P \left(h^{(t)}_i \,|\, \mu_k^{(t-1)},\,\Sigma_k^{(t-1)}\right)^\beta}
    {\sum_{k'=1}^{K}\pi_{k'}^{(t-1)}P \left(h^{(t)}_i \,|\, \mu_{k'}^{(t-1)},\, \Sigma_{k'}^{(t-1)}\right)^\beta}.
\end{equation}
Here, $\gamma_{ik}^{(t)}$ denotes the soft assignment of latent vector $h^{(t)}_i = f^{(t)}_\phi(v_i)$ from the teacher network to the $k$-th Gaussian component. Intuitively, it reflects how well the $k$-th component's distribution explains $h^{(t)}_i$. To further enhance prototype utilization, particularly when employing a large number of components $K$, we introduce an annealing mechanism controlled by a smoothing factor $\beta \in [0,1]$~\cite{ueda1998deterministic}, which modulates the sharpness of the responsibilities during training.

% TODO: Continue writing from here, transition into that this is our expectation step and introduce the weighted forgetting factor of Celaya (2015).

Following the assignment of responsibilities, the expectation step utilizes these values to compute the intermediate sufficient statistics for the current timestep necessary to update the mixture's sufficient statistics. Specifically, at each time step, the intermediate sufficient statistics are calculated as:
\begin{equation}
\label{eq:suff_stats}
    \tilde{S}^{(t)}_k = \left\{\tilde{S}_{k,\pi}^{(t)},\; \tilde{S}_{k,\mu}^{(t)},\; \tilde{S}_{k,\Sigma}^{(t)}\right\} = \left\{\sum_{i=1}^{VB}\gamma_{ik}^{(t)},\; \sum_{i=1}^{VB}\gamma_{ik}^{(t)}h_i^{(t)},\; \sum_{i=1}^{VB}\gamma_{ik}^{(t)}h_i^{(t)}h_i^{(t)^T}\right\}.
\end{equation}
These intermediate statistics are then used to update the sufficient statistics of the mixture using a weighted moving average:
\begin{equation}
\label{eq:suff_stats_ema}
{S}^{(t)}_k = 
\begin{cases} 
\eta^{\hat{\gamma}_k} {S}^{(t-1)}_k + (1-\eta^{\hat{\gamma}_k})\tilde{S}^{(t)}_k & \text{if } t > 1, \\
\tilde{S}^{(1)}_k\footnotemark  & \text{otherwise}.
\end{cases}
\end{equation}
\footnotetext{See Appendix~\ref{app:suff_stat_init} for a detailed discussion of the initialization strategy for the sufficient statistics.}
Here, $\eta \in [0,1]$ is a forgetting factor, controlling the influence between new and past information. When using a large number of prototypes $K$ the mixture's components will receive sparse updates, thus, the forgetting factor $\eta$ will tend to push the sufficient statistics towards zero. To circumvent this issue, we introduce a responsibility based forgetting mechanism~\cite{celaya2015online} through the incorporation of the expectation of the responsibilities over the batch dimension $\hat{\gamma}_k = \frac{1}{VB}\sum_i^{VB}\gamma_{ik}$. By raising the forgetting factor to the power of $\hat{\gamma}_k$, components with higher expected responsibility receive more aggressive updates, whereas those with lower responsibilities retain a larger fraction of their previous statistics, thereby preventing the sufficient statistics to be pushed towards zero.

 
Given the updated sufficient statistics, we proceed to the maximization step of the EM algorithm, wherein the GMM parameters $\Psi$ are updated. This step updates the mixture weights, means, and covariances by computing their maximum likelihood estimates based on the current sufficient statistics:
\begin{equation}
\label{eq: maximization_step}
    \pi_k^{(t)}=\frac{S_{k,\pi}^{(t)}}{\sum_{k'=1}^K S^{(t)}_{k', \pi}},  \quad
    \mu_k^{(t)}= \frac{S_{k,\mu}^{(t)}}{S_{k,\pi}^{(t)}}, \quad
    \Sigma_k^{(t)}= \frac{S_{k,\Sigma}^{(t)}}{S_{k,\pi}^{(t)}} - \frac{S_{k,\mu}^{(t)}S_{k,\mu}^{(t)^T}}{S_{k,\pi}^{(t)}S_{k,\pi}^{(t)}}.
\end{equation}
In the context of our prototypical SSL framework, the updated means $\mu_k$ serve as prototypes for the latent assignments, i.e. $\mu_k=c_k$ for $k=1,\ldots,K$. It is important to note that this maximization step is performed prior to the encoder’s optimizer step, ensuring that the prototypes reflect the most recent assignment statistics before any encoder parameters are updated. 

==> sections/4_case_study.tex <==
\section{Experiments}
\label{experiments}
\subsection{Uniqueness of prototypes under different thresholds}
\begin{table}[ht]
    \centering
    \caption{Unique prototypes for different values of $\epsilon$. \textbf{NOTE}: Turn this into a figure.}
    \label{tab:protos_under_diff_eps}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l l l l l l l l}
        \toprule
        \textbf{Model} & \textbf{Arch} &  \textbf{Objective} &$\boldsymbol{\epsilon = 0.50}$ & $\boldsymbol{\epsilon = 0.25}$ & $\boldsymbol{\epsilon = 0.10}$ & $\boldsymbol{\epsilon = 0.05}$ & $\boldsymbol{\epsilon = 0.025}$ \\
        \midrule
        DINO      & ResNet-50 & Instance &442 (0.7\%) & 791 (1.2\%) & 895 (1.3\%) & 948 (1.4\%) & 1012 (1.6\%) \\
        CARP      & ResNet-50 & Instance &490 (0.7\%) & 1609 (2.5\%) & 5031 (0.8\%) & 10312 (15.7\%) & 19417 (29.6\%) \\
        CAPI & ViT-L/16 & Dense & 9214 (56.2\%) & 14488 (88.4\%) & 16183 (98.8\%) & 16370 (99.9\%) & 16383 (100\%) \\
        CARP w/ decoupling & ResNet-50 & Instance & 65536 (100\%) & 65536 (100\%) & 65536 (100\%) & 65536 (100\%) & 65536 (100\%) \\
        \bottomrule
    \end{tabular}%}
    }
\end{table}

\subsection{Training dynamics}
Although previous studies have examined partial prototype collapse, they have focused exclusively on its manifestation at the end of training \citep{govindarajan2023dino, Govindarajan_2024_BMVC}, and its interaction with the dynamics of training itself remains unclear. To address this and gain deeper insight into the relationship between prototype collapse and training dynamics, we track the number of unique prototypes in use and the linear evaluation accuracy on ImageNet-1k \citep{deng2009imagenet} over the first 100 epochs for CARL, CARP, DINO, DINO + KoLeoProto, and DINO + Subsampling, as shown in Figure \ref{fig:protos-acc-two-subplots}.

A first observation is that partial prototype collapse emerges very early in training: after only 10 epochs, nearly two-thirds of the prototypes have already collapsed. Introducing the KoLeo-Proto (KP) regularizer proves effective at maintaining prototype diversity, underscoring its role as a strong collapse-prevention mechanism. While DINO+KP exhibits a modest drop in accuracy during the early stages of training, this effect diminishes over time, and the final model slightly outperforms vanilla DINO. This suggests that preserving higher prototype diversity throughout training ultimately leads to stronger representations in the converged model.

Another noteworthy observation is that CARP, as hypothesized, is far less prone to prototype collapse than the baseline CARL. By the end of training, CARL retains only about $0.2\%$ of its initialized prototypes as unique, whereas CARP preserves $91.7\%$. This difference is also reflected in linear evaluation performance: CARP consistently outperforms CARL both early and late in training. While these gains cannot be attributed solely to prototype uniqueness—training stability likely plays a significant role—they nevertheless amount to a substantial margin of roughly 3.5 percentage points in linear accuracy by the end of training.

Lastly, we observe that DINO with Subsampling (SS) does alleviate the partial prototype collapse problem to some extent. However, the resulting increase in prototype diversity is accompanied by a considerable drop in accuracy, likely because only a quarter of the prototypes are updated at each iteration, reducing the overall training signal. This suggests that the SS strategy may be more beneficial in settings with uncurated, imbalanced data than on curated, uniform datasets such as ImageNet-1k.

\begin{figure}[tb]
\centering
\resizebox{\linewidth}{!}{%
\begin{tikzpicture}
\pgfplotsset{compat=1.18}

% ---------------------- DATA TABLES ----------------------
\pgfplotstableread[row sep=\\,col sep=space]{
epoch  dino   dinokp  dinoss  carl   carp \\
0      65536  65536   65536   65536  65536 \\
10     23249  65534   36567   65527  64207 \\
20     16826  65536   19107     522  62752 \\
30     14033  65523   13565     145  62018 \\
40      6431  65285   10130     141  61615 \\
50      4734  65021    7531     141  61316 \\
60      3522  64593    5805     141  60944 \\
70      2812  64150    4643     141  60561 \\
80      2490  63883    4029     141  60256 \\
90      2347  63436    3741     141  60102 \\
100     2338  63365    3682     141  60082 \\
}\prototbl

\pgfplotstableread[row sep=\\,col sep=space]{
epoch  dino   dinokp  dinoss  carl   carp \\
0      0      0       0       0      0 \\
10     37.49  36.14   42.78   nan    46.25 \\
20     56.82  55.75   49.86   nan    59.12 \\
30     62.46  62.36   53.69   nan    63.10 \\
40     64.71  64.91   55.80   nan    65.04 \\
50     65.63  66.20   57.34   nan    66.53 \\
60     66.72  67.49   58.54   nan    67.44 \\
70     67.70  68.65   59.34   nan    68.49 \\
80     68.93  70.08   59.91   nan    68.00 \\
90     69.72  70.77   59.99   nan    68.57 \\
100    70.00  70.91   60.02   65.03  68.66 \\
}\acctbl

% ---------------------- PLOTS ----------------------
\begin{groupplot}[
  group style={group size=2 by 1, horizontal sep=10ex},
  height=6cm, width=8.5cm,
  xmin=0, xmax=100,
  xtick={0,10,20,30,40,50,60,70,80,90,100},
  scaled x ticks=false,
  grid=both,
  xmajorgrids=true, ymajorgrids=true, minor grid style={opacity=0.2},
  yminorgrids=false,
  every axis plot/.append style={line width=1.4pt, mark=none},
  tick style={semithick},
  label style={font=\small},
  tick label style={font=\small},
  unbounded coords=jump
]

% --- (1) Unique prototypes (log scale) ---
\nextgroupplot[
  title={Unique prototypes over epochs},
  xlabel={Epoch}, ylabel={\# unique prototypes},
  ymode=log, log basis y=10,
  ymin=100, ymax=70000,
  ytickten={2,3,4},
  legend style={
    font=\scriptsize,
    at={(0.02,0.98)}, anchor=north west,
    fill=white, fill opacity=0.8, draw=none,
    /tikz/every even column/.style={column sep=6pt},
  },
  legend columns=2,
  legend to name=protos-acc-lgd,
]
\addplot+ table[x=epoch,y=dino]   {\prototbl};
\addplot+ table[x=epoch,y=dinokp] {\prototbl};
\addplot+ table[x=epoch,y=dinoss] {\prototbl};
\addplot+ table[x=epoch,y=carl]   {\prototbl};
\addplot+ table[x=epoch,y=carp]   {\prototbl};
\legend{DINO, DINO + KP, DINO + SS, CARL, CARP}

% --- (2) Accuracy (broken y-axis style) ---
\nextgroupplot[
  title={Accuracy over epochs (ImageNet)},
  xlabel={Epoch}, ylabel={Top-1 (\%)},
  ymin=40, ymax=75,           % << focus region
  ytick={40,50,60,70},        % ticks only in zoom range
  scaled y ticks=false,
  legend style={
    font=\scriptsize,
    at={(0.02,0.98)}, anchor=north west,
    fill=white, fill opacity=0.8, draw=none,
    /tikz/every even column/.style={column sep=6pt},
  },
  legend columns=5,
  unbounded coords=jump,
  % little diagonal lines at y-axis to indicate break:
  axis line style={-},        % draw axes manually
  clip marker paths=true,
  extra description/.code={
    \draw[black,thick] (rel axis cs:0,0) -- ++(0.2cm,-0.2cm);
    \draw[black,thick] (rel axis cs:0,1) -- ++(0.2cm,0.2cm);
  },
]
\addplot+ table[x=epoch,y=dino]   {\acctbl};
\addplot+ table[x=epoch,y=dinokp] {\acctbl};
\addplot+ table[x=epoch,y=dinoss] {\acctbl};
\addplot+ table[x=epoch,y=carl]   {\acctbl};
\addplot+ table[x=epoch,y=carp]   {\acctbl};
%\legend{DINO, DINO + KP, DINO + SS, CARL, CARP}
\end{groupplot}
\node[below] at ($(group c1r1.south)!.5!(group c2r1.south)$) {\pgfplotslegendfromname{protos-acc-lgd}};
\end{tikzpicture}}
\caption{(a) Number of unique prototypes over epochs. Prototypical methods without explicit diversity mechanisms (e.g., DINO and CARL) exhibit substantial prototype collapse early in training.
(b) Linear evaluation accuracy on ImageNet-1k. Higher prototype diversity generally correlates with stronger final performance, though some methods (e.g., DINO + KP) imposes a cost of slower early convergence.}
\label{fig:protos-acc-two-subplots}
\end{figure}

\subsection{Effect of protototype diversity across head, medium and tail classes}
\textbf{Todos:}
\begin{enumerate}
    \item First, showcase linear probe accuracy on methods pre-trained on long-tailed datasets. We'll show that DINO+KP and CARP outperform DINO and CARL. MAPL will perform worse, explain this limitation with a hypothesis that MAPL likely is not good on modeling tail-classes due to the mixture formulation.
    \item Go more granular, bucket tail-classes as classes with ($\leq$20 instances per class) medium-shot classes ($<20\leq100$ instances per class) head-classes (100< instances per class) \textbf{TODO:} lookup in literature which are the headclasses, tail-classes etc. for iNat. 
\end{enumerate}

\begin{table}[t]
\centering
\caption{Performance comparison on the iNaturalist 2018 dataset. Results are reported as Top-1 accuracy (\%) for different class splits (Many, Medium, Few, All).}
\begin{tabular}{lcccc}
\toprule
Methods & Head ($>100$) & Medium ($\leq 100\ \& > 20$)& Tail ($\leq 20$)& All \\
\midrule
DINO      &  -- & -- & -- & -- \\
DINO+KP   &  -- & -- & -- & -- \\
CARL      &  -- & -- & -- & -- \\
CARP      &  -- & -- & -- & -- \\
\rowcolor{highlight} MAPL      &  -- & -- & -- & -- \\
\bottomrule
\end{tabular}
\label{tab:inat_dino}
\end{table}


\subsection{Prototype Utilization}
\label{case_study:prototype_util}
% \begin{definition}[Partial prototype collapse]
% Consider the set $W = \{\bmu_k : k=1,...,K\}$ of $K$ prototype vectors, $\bmu_k$ such that $\Vert \bmu_k \Vert = 1$. A \emph{partial prototype collapse} (of degree $M$ and $\epsilon$ distance) is said to have occurred if there exists a set of $M$ disjoint partitions of prototype vectors $V_m \subset W$, $m = 1, ..., M$, and $M$ representative prototype vectors $\bv_m \in V_m$, such that for all $m = 1, ..., M$, 
% $1-\bv_m^{\mathsf{T}}\bmu_j < \epsilon$, for all $\bmu_j \in V_m$.
% The set of $M$ \emph{unique prototypes} is defined as $U = \{ \bv_m \}_{m=1}^M$. For each representative prototype, the \emph{redundancy factor} $r_m$ is defined as the size of the corresponding set partition, $r_m = |V_m|$.
% \end{definition}

\begin{definition}[Prototype Utilization]
Consider a prototype set $C=\{c_k : k=1,\dots,K\}$ and the prototype probability assignments 
$p(z_i)\in\mathbb{R}^{K}$ obtained from similarities 
$z_i = \text{cos}(C, h_i)$ where $\text{cos}(\cdot,\cdot)$ represents the cosine similarity. 
Given a threshold $\gamma \in (0,1)$ and a minimum support $m \geq 1$. 
A prototype $c_k$ is said to be \emph{utilized} if it is assigned with probability at least $\gamma$ 
for at least $m$ representations in the set of images, i.e. $
\mathcal{U}_k= \sum_{i=1}^N  \mathbf{1}\{\,p_k(z_i) \geq \gamma\,\} \;\; \geq m.
$
\end{definition}


\begin{table}[ht]
\centering
\caption{Unique Prototypes vs. Prototype Utilization}
\resizebox{\textwidth}{!}{%
\begin{tabular}{l l r r r}
\toprule
Method & Training Dataset & Unique Prototypes & Proto. Util. wrt. Initial Protos (\%) & Proto. Util. wrt. Unique Protos (\%) \\
\midrule
DINO    & ImageNet-1k   & 2,338 (3.5\%)   & 1.9  & 88.1 \\
DINOv2  & ImageNet-21k  & 6,932 (2.7\%)  & 2.1  & 84.5 \\
Franca  & ImageNet-21k  & 8,309 (3.2\%)  & 2.6  & 86.5 \\
CARP    & ImageNet-1k   & 19,417 (29.6\%) & 23.7 & 89.2 \\
\rowcolor{highlight}
Ours    & ImageNet-1k   & 65,536 (100\%)  & 53.0 & 53.0 \\
\bottomrule
\end{tabular}%
}
\end{table}


==> sections/5_results.tex <==
\section{Main Results}
\subsection{Linear Classification}
\subsubsection{Pre-training on ImageNet-1k}
As MAPL only incorporates an instance-based loss we compare with those in our results in \ref{}. For additional results with methods incorporating dense-loss and other SSL formulations, please refer to the appendix. 
\begin{table}[tb]
\centering
\caption{ImageNet evaluation results for various prototypical SSL methods and architectures. Unique prototypes at $\epsilon=0.025$ and their percentage relative to initialized prototypes are reported. \(^\dagger\) Results computed by us using the officially released pre-trained models.}
\label{tab:imagenet_results}
\footnotesize
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  colspec={*{3}{l} r rr rr},
  %row{2,3} = {fg=gray},
  row{6,8,12,15} = {bg=highlight},
  column{5} = {rightsep=0pt},
  column{6} = {leftsep=0pt}
}
\toprule
\textbf{Method} & \textbf{Backbone} & \textbf{Dataset}& \textbf{Epochs} & \SetCell[c=2]{r}{\textbf{Unique Protos.}} & &\textbf{k-NN (\%)} & \textbf{Linear (\%)} \\
DINO   \citep{caron2021emerging}    & RN-50 & ImageNet-1k& 400 & 1012 & (1.6\%)\(^\dagger\) & 67.5 & 75.3 \\
SWAV  \citep{caron2020swav}     & RN-50 & ImageNet-1k & 400 & 1761 & (58.7\%)\(^\dagger\)& 65.0 \(^\dagger\) & 74.6\\
DeepCluster-v2  \citep{caron2020swav}     & RN-50 & ImageNet-1k & 400 & --& --&  TBD \(^\dagger\) & 74.3\\
CARP \citep{silva2023carp}     & RN-50 & ImageNet-1k & 400 & 19417 & (29.6\%)\(^\dagger\) & 67.7 & 75.3 \\
\METHODNAME       & RN-50 & ImageNet-1k & 400 & 65536 & (100\%) &  69.1   &  --   \\
\midrule
DINO  \citep{caron2021emerging}     & ViT-S/16 & ImageNet-1k & 300 &   & -- &72.8 & 76.2 \\
\METHODNAME       & ViT-S/16 & ImageNet-1k & 300 & 65536 & (100\%)   &  74.1   & 76.4 \\
\midrule
MSN \citep{assran2022msn} & ViT-S/16 & ImageNet-1k & 600  & 810  & (79.1\%)\(^\dagger\) & -- & 76.9 \\
DINO  \citep{caron2021emerging}    & ViT-S/16 & ImageNet-1k & 800 &  & -- &  74.5 & 77.0 \\
DINO-vMF  \citep{govindarajan2023dino}    & ViT-S/16 & ImageNet-1k & 800 &  & -- &  74.7 & 77.0 \\
\METHODNAME       & ViT-S/16 & ImageNet-1k & 800 & 65536 & (100\%)   &  75.3   & -- \\
 \midrule
DINO  \citep{caron2021emerging}     & ViT-B/16 & ImageNet-1k & 400 &   & -- & 76.1 & 78.2 \\
DINO-vMF  \citep{govindarajan2023dino}     & ViT-B/16 & ImageNet-1k & 400 &   & -- & 77.4 & 78.8 \\
\METHODNAME       & ViT-B/16 & ImageNet-1k & 400 & 65536 & (100\%)   &  76.7   & -- \\
\bottomrule
\end{tblr}
} 
\end{table}


\subsubsection{Pre-training with iNaturalist-2018}

\begin{table}[tb]
\centering
\caption{iNat-2018 classification accuracies with full data. \(^\dagger\)Results retrieved from \cite{Govindarajan_2024_BMVC}.}
\label{tab:imagenet_results}
\footnotesize
\resizebox{\linewidth}{!}{%
\begin{tblr}{
  colspec={l r  r rr},
  row{9,13} = {bg=highlight},
  column{2} = {rightsep=0pt},
  column{3} = {leftsep=0pt}
}
\toprule
\textbf{Method}& \SetCell[c=2]{r}{\textbf{Unique Protos.}} &   & \textbf{Linear (\%)} & \textbf{Fine-tuned (\%)} \\
\midrule 
\textbf{ViT-Small/16} & & & & \\
DINO-vMF\(^\dagger\)    \citep{govindarajan2023dino}       & 1380 & (2.1\%) &  49.7 & 68.5 \\
iBOT-vMF\(^\dagger\)     \citep{govindarajan2023dino}       & 1804 & (22.0\%) &  50.1 & 69.4 \\
iBOT-vMF (kd)\(^\dagger\)  \citep{govindarajan2023dino, oquab2024dinov}      & 1843 & (22.5\%)  & 50.5 & 69.1 \\
iBOT-vMF (kp)\(^\dagger\)  \citep{Govindarajan_2024_BMVC}      & 7895 & (96.4\%) & 51.1 & 69.3 \\
MSN ($\lambda=1$)\(^\dagger\)  \citep{assran2022msn} & 3363 & (41.3\%) &  53.8 & 63.5 \\
PMSN ($\lambda=5$)\(^\dagger\)  \citep{assran2023pmsn} & 3005 & (36.9\%)&  41.8 & 64.2 \\
\METHODNAME       & 65536 & (100\%) &  TBD & 71.7 \\
\midrule 
\textbf{ViT-Base/16 }& & & & \\
iBOT-vMF (kd)\(^\dagger\)  \citep{govindarajan2023dino, oquab2024dinov} &  1634 & (19.9\%) &  50.4 & 73.3 \\
iBOT-vMF (kp)\(^\dagger\)  \citep{Govindarajan_2024_BMVC} &  7573 & (92.4\%) &  51.4 & 74.0 \\
\METHODNAME       & 65536 & (100\%) & TBD & 71.3  \\
\bottomrule
\end{tblr}}
\end{table}



\subsection{Transfer Learning}

\begin{table}[tb]
  \centering
  \caption{Transfer learning results for various prototypical methods. We follow \cite{ericsson2021well} transfer learning protocol.}
  \label{tab:laionet_results}
\resizebox{\linewidth}{!}{%}
\begin{tblr}{
    colspec = {l  rr *{13}{r}},
    row{8,12} = {bg=highlight},
    column{3} = {rightsep=0pt},
    column{4} = {leftsep=0pt}
  }
  \toprule
  Method & Epochs &
  \SetCell[c=2]{c}{Unique Protos.} & &
  Aircr &  C101 & Cars & CF10 & CF100 & DTD & Flower &
  Food & Pets & SUN & VOC & Avg \\
  \midrule
  \textbf{ResNet-50} & \SetCell[c=15]{l}{} \\
  SWaV~\citep{caron2020swav}  & 400  & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD  \\ 
  SWaV~\citep{caron2020swav}  & 800  & TBD & (--\%) & 54.04 & 90.84 & 54.06 & 93.99 & 79.58 & 77.02 & 94.62 & 76.62  & 87.60 & 65.58 & 83.68 & 77.97 \\ 
  DeepClusterv2\citep{caron2020swav} & 400  & -- & -- & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD  \\ 
  DeepClusterv2\citep{caron2020swav} & 800  & -- & -- & 54.49 & 91.33 & 58.60 & 94.02 & 79.61 & 78.62 & 94.72 & 77.94 & 89.36 & 65.48 & 83.94 & 78.92 \\ 
  DINO~\citep{caron2021emerging}  & 400  & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\ 
  MAPL (Ours)   & 400  & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD  \\
  \midrule
  \textbf{ViT-Small} & \SetCell[c=15]{l}{} \\
  DINO~\citep{caron2021emerging}  &  800 & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
  MSN~\citep{assran2022msn} &  600    & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD \\
  MAPL (Ours)     & 800                      & TBD & (--\%) & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD & TBD  \\
  \bottomrule
\end{tblr}}
\end{table}


==> sections/6_ablations.tex <==
\section{Ablations}
\label{sec:ablations}
\subsection{Importance of the Different Components}
\begin{table}[tb]
\centering
\caption{Ablation study of model components.}
\label{tab:ablation}
\begin{tabular}{lccccccc}
\toprule
WDFF & Entropy Reg. & Partitioning & Annealing & Re-Init. & Rescaling & k-NN & Lin. \\
\midrule
 \xmark & \checkmark &  \checkmark  & \checkmark & \checkmark & \checkmark & 0.1 & 0.1 \\ 
 \checkmark & \xmark & \checkmark & \checkmark & \checkmark & \checkmark & 0.1 & 0.1 \\
 \checkmark & \checkmark & \xmark & \checkmark & \checkmark & \checkmark & 0.1 & 0.1 \\
 \checkmark & \checkmark & \checkmark & \xmark & \checkmark & \xmark & - & 71.65\\
 \checkmark & \checkmark & \checkmark & \xmark & \checkmark & \checkmark & - & 71.97 \\
  \checkmark & \checkmark & \checkmark & \xmark & \xmark & \xmark & - & 71.99 \\
  \checkmark & \checkmark & \checkmark & \checkmark  & \xmark & \xmark & - & 72.12 \\
\rowcolor{highlight} \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & \checkmark & - & 72.25 \\
\bottomrule
\end{tabular}
\end{table}

\subsection{The Effect of the Batch Size}
\begin{table}[]
    \centering
    \begin{tabular}{ccccc}
    \toprule
         Batch Size & 256 & 512 & 1024 & 2048   \\
        \midrule
     k-NN &  67.28\% & 69.28\% & 69.37\% & 47.32\% \\
    \bottomrule
    \end{tabular}
    \caption{Larger batch size benefits MAPL until 1024 batch size but then deteriorates.}
    \label{tab:bs_ablation}
\end{table}

==> sections/7_related_work.tex <==
\section{Related Work}
\subsection{Prototypical Self-Supervised Learning}
One of the most prominent families of self-supervised learning methods for vision-only encoders is based on prototypes. Early approaches relied on applying K-means to all latent representations once per epoch \citep{caron2018deep}. Later work introduced online formulations for learning prototypes, with a common strategy being the use of the Sinkhorn-Knopp algorithm \citep{cuturi2013sinkhorn} to address the cluster assignment problem \citep{caron2020swav, asano2019self}. More recent work prototypical frameworks borrow a teacher-student formulation as introduced in BYOL \citep{grill2020bootstrap}, where the teacher is an exponential moving average of the student's weights  
CARL, CARP \citep{silva2022carl, silva2023carp}, DeepCluster \citep{caron2018deep}, SWaV \citep{caron2020swav},DINO \citep{caron2021emerging}, iBOT \citep{zhou2022image}, DINOv2 \citep{oquab2024dinov}, DINOv3 \citep{dinov3}, WebDINO \citep{fan2025webdino}, DINO-vMF \citep{govindarajan2023dino}, MSN, PMSN \citep{assran2022msn, assran2023pmsn}. 
\subsection{Prototype utilization}
Partial Collapse Paper \citep{Govindarajan_2024_BMVC}, Subsampling method\citep{wen2024makes}, Ensemble-Head paper \citep{ruan2023weighted}, implicit regularization to enhance prototypical utilization \citep{silva2023carp}. 

==> sections/8_conclusion.tex <==
\section{Conclusion}
